MixtureGrowth: Growing Neural Networks by Recombining Learned Parameters

Most deep neural networks are trained under fixed network architectures and require retraining when the architecture changes. If expanding the network's size is needed, it is necessary to retrain from scratch, which is expensive. To avoid this, one can grow from a small network by adding random weights over time to gradually achieve the target network size. However, this naive approach falls short in practice as it brings too much noise to the growing process. Prior work tackled this issue by leveraging the already learned weights and training data for generating new weights through conducting a computationally expensive analysis step. In this paper, we introduce MixtureGrowth, a new approach to growing networks that circumvents the initialization overhead in prior work. Before growing, each layer in our model is generated with a linear combination of parameter templates. Newly grown layer weights are generated by using a new linear combination of existing templates for a layer. On one hand, these templates are already trained for the task, providing a strong initialization. On the other, the new coefficients provide flexibility for the added layer weights to learn something new. We show that our approach boosts top-1 accuracy over the state-of-the-art by 2-2.5% on CIFAR-100 and ImageNet datasets, while achieving comparable performance with fewer FLOPs to a larger network trained from scratch. Code is available at https://github.com/chaudatascience/mixturegrowth.

==> figs/FIG_create.tex <==
%Figure 1:
%Run 
`%/projectnb/ivc-ml/piotrt/gradmax/growneuron/jupyter_analysis/Figure1 Incremental.ipynb`
% ver2: use grow=63, and add ours (ens.): '/projectnb/ivc-ml/chaupham/anytime/param_share/incremental_training/Figure1_Incremental_v2.ipynb'

%%Fig 2 (different growth points): 
% Jupyter notebook: /projectnb/ivc-ml/chaupham/anytime/param_share/incremental_training/different_growth.ipynb

%%% Fig 3, 4
% '/projectnb/ivc-ml/chaupham/anytime/param_share/incremental_training/different_growth_v2.ipynb'


%Horizontal Figures: https://docs.google.com/presentation/d/1eVcaP4IL1Sp9RR9S6Oyuqik_LTJtBUNSh9hE0FhSNFg/edit?usp=sharing. 

%Vertical Figures: https://docs.google.com/presentation/d/15nmpGt5k8qWiIkl2zYgAQkJwf1h2C7k1KvoJPxJO29s/edit#slide=id.g184a01f20cc_0_165

==> tables/baselines_gradmax_schedule.tex <==
\setlength{\tabcolsep}{2pt} % Default value: 6pt
\begin{table*}[t]
% \resizebox{1.08\textwidth}{!}{
\centering
\caption{\textbf{Network growing comparison on CIFAR-100}. \textbf{(a)} Using the long growing schedule used by the authors of GradMax; 
\textbf{(b)} provides \OurMethod{} performance using multiple growth fashion (depicted in Fig. \ref{fig:multi_growth}), where it achieves the same performance as the baselines with fewer FLOPs;
\textbf{(c)} \OurMethod{} with single growth for reference.} 
\begin{tabular}{rlcc} 
\toprule
 & Method & Top-1 Acc.  &  FLOPs Norm   \\
 \midrule
 \textbf{(a)} & Random & 79.12\% &  0.77X \\
 & Firefly~\cite{wu2020firefly} & 78.94\% &  0.77X \\
 & GradMax~\cite{evci2022gradmax} & 79.24\% &  0.77X \\  
 \midrule
 % Note: 0.77X due to we train with a longer schedule (200 epochs). Before, this was 1.54X instead.
 \textbf{(b)} & \OurMethod{} w/ multiple growth & 79.13\%   & 0.45X \\  
  \textbf{(c)} & \textbf{\OurMethod{}} & \textbf{81.50\%}   & 0.45X \\
 \bottomrule
\end{tabular}
\label{table:gradmax_schedule_multi}
\hfill
\end{table*}

==> tables/coef_init.tex <==
\setlength{\tabcolsep}{20pt} % Default value: 6pt
\begin{wraptable}{r}{0.60\textwidth}
\caption{\textbf{Ablation on coefficient initialization methods} (described in Section~\ref{sec:tiling}) for \OurMethod{}. We report average Top-1 accuracy over 3 runs on CIFAR-100. Orthogonal initializations perform best, suggesting that it is important for instantiated weights to be independent to encourage diversity.
}
\begin{tabular}{lc} 
 \toprule
 Method & Top-1 Accuracy    \\ [0.5ex] 
 \midrule
 Random coefficients  & 81.41\%  \\ 
 Coefficient copying & 79.05\% \\ 
 Orthogonal coefficients & \textbf{81.50}\%   \\
  \bottomrule
\end{tabular}

\label{table:coef_init}

\end{wraptable}


==> tables/coeff_copy_orthogonal_random.tex <==

\begin{table*}[t]
\centering
\begin{tabular}{lr} 
 \toprule
 Method & Top-1 Accuracy    \\ [0.5ex] 
 \midrule
 Random coefficients  & 81.41\%  \\ 
 Coefficient copying & 79.05\% \\ 
 Orthogonal coefficients & \textbf{81.50}\%   \\
  \bottomrule
  \end{tabular}
\caption{\textbf{Ablation on alpha-coefficient initializations:} Accuracy averaged over three runs of \OurMethod{} with different coefficient initialization methods (described in Section~\ref{sec:tiling}) on CIFAR-100. We find orthogonal initializations to perform best, suggesting that it is important for instantiated weights to be independent to encourage diversity. }
\label{table:cifar100_coeff}
\end{table*}



==> tables/data_growth.tex <==
\setlength{\tabcolsep}{2pt} % Default value: 6pt
\begin{table*}[t]

\centering
\caption{Network growing comparison under data growth setting}

% \resizebox{\textwidth}{!}{

\begin{tabular}{rlccc:ccc} 
\toprule
 & Method & CIFAR-10~\cite{Krizhevsky09learningmultiple} & CIFAR-100~\cite{Krizhevsky09learningmultiple}  &  FLOPs Norm & ImageNet~\cite{deng2009imagenet} &  FLOPs Norm\\ 

 & Net2Net\cite{chen2015net2net} & 96.31 \% &77.53\% & 0.45X  & -\% & 0.35X\\
   & Random & 92.22\% & 71.46\% & 0.45X  &-\% & 0.35X\\
 & Firefly~\cite{wu2020firefly} & 91.38\% & 71.68\% &  0.45X  & -\% & 0.35X  \\
 & GradMax~\cite{evci2022gradmax} & 91.90\% &71.53\% & 0.45X & -\% & 0.35X\\  
  & \OurMethod{} w/o fusion & \% & 74.47\% &  0.45X & -\% & 0.35X\\
 & \textbf{\OurMethod\ (ours)} & \textbf{96.49\%} & \textbf{79.58\%} &  0.45X & \textbf{-\%} & 0.35X\\
 
   
 \bottomrule
\end{tabular}
% }

\label{table:data_growth}

\end{table*}

==> tables/different_growth.tex <==

% \begin{table}[t]
% \centering
% \begin{tabular}{rlcc} 
% \toprule
%  Method & Top-1 Acc. &  FLOPs Norm   \\
%  \midrule
%  Horizontal growth & 78.760\% &  3.759e+11 \\
%  Vertical growth & 79.260\% &  3.769e+11 \\

%  \bottomrule
% \end{tabular}
% \caption{Comparison different growth method of \OurMethod{} on CIFAR-100 using WRN-28-10 architecture. We report average accuracy of three runs for each method. 
% }
% \label{table:horizontal_vertical}
% \end{table}
% % Horizontal 79.10, 79.05, 79.37 FLOPs 3.792e+11



% max_params = 36500000

CIFAR100: 
[200, 150, 100, 90, 80, 70, 60, 50, 40, 30, 20][79.630, 79.130, 79.540, 79.120, 79.120, 79.660, 79.120, 79.260, 79.490, 78.760, 78.680]


CIFAR10: 
[200, 150, 100, 90, 80, 70, 60, 50, 40, 30, 20][95.670, 95.670, 95.720, 95.670, 95.530, 95.680, 95.710, 95.770, 95.550, 95.520, 95.720]
[3.832e+11, 3.811e+11, 3.791e+11, 3.786e+11, 3.778e+11,3.773e+11, 3.769e+11, 3.764e+11, 3.759e+11, 3.759e+11]

==> tables/diffrent_num_params.tex <==
%%%%%%% Not used. Replaced by a graph

% \begin{table}[t]
% \centering
% \caption{Results of MixtureGrowth on CIFAR-100 using a WRN 28-10 as the Target network with different growth points. Overall, the result is not very sensitive to the growth point, except for the growth at the very end of training. This allows us to minimize training FLOPS while retaining high accuracy.}
% \label{table:cifar100}
% \begin{tabular}{|c|cc|} 
%  \hline
%  Grow at & Top-1 & FLOPs Norm   \\ [0.5ex] 
%  \hline
%  18 & 79.35\% &  0.93X  \\ 
%  \hline
%  28 & 79.45\% & 0.88X  \\ 
%  \hline
%  38 & 79.27\% & 0.83X  \\
%  \hline
% 49 & 79.14\% & 0.77X  \\
%  \hline
%  63 & 79.21\% & 0.70X \\
%  \hline

% \end{tabular}
% \end{table}

==> tables/lower_FLOPS_imagenet.tex <==

\begin{table}[t]
\centering
\begin{tabular}{rlcc} 
\toprule
 Method & Top-1 Acc. &  FLOPs Norm   \\
 \midrule
 Target match 49 & 76.12\% &  0.55X \\
 Target match 54 & 76.33\% &  0.60X \\
 Target match 58 & 76.58\% &  0.65X \\
 Target match 63 & 76.60\% &  0.70X \\
\midrule
 \OurMethod{} grow 83 & 74.04\% &  0.55X \\
 \OurMethod{} grow 74 & 74.72\% &  0.60X \\
 \OurMethod{} grow 65 & 75.53\% &  0.65X \\
 \OurMethod{} grow 56 & 76.09\% &  0.70X \\

 \bottomrule
\end{tabular}
\caption{Comparison growth methods under different FLOPs budgets on Imagetnet. 
}
\label{table:horizontal_vertical}
\end{table}



==> tables/main_imagenet.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{rlcccc} 
\toprule
 & Method & ImageNet~\cite{deng2009imagenet} &  FLOPs Norm\\ 
\midrule
 \textbf{(a)} & Target &  76.49\% & 1.00X \\ 
 % \hline
 & Target Match & 73.85\% & 0.36X \\ 
 % \hline
 & Seed & 72.48\% & 0.25X \\
 %%% train seed model in 280 epochs
  & Seed Match & 72.89\% & 0.36X \\
  \midrule
 \textbf{(b)} & Random & 71.47\% & 0.36X \\
 & Firefly~\cite{wu2020firefly}  & 71.30\% & 0.36X \\
 & GradMax~\cite{evci2022gradmax} & 71.73\% & 0.36X \\  
 & \textbf{\OurMethod\ (ours)} & \textbf{74.35\%} & 0.36X \\
 \bottomrule
\end{tabular}
\caption{Network growing comparison using top-1 accuracy averaged over three runs for fixed training FLOP budget. \textbf{(a)} reports the performance of training the large (post-growth) \emph{Target} network architecture from scratch (WRN-28-10 for both CIFAR datasets and ResNet-50 for ImageNet), as well as performance of the small (pre-growth) \emph{Seed} architecture (WRN-28-5 for both CIFAR datasets and a ResNet-50 with half the channels as the large network for ImageNet).  \textbf{(b)} reports the performance of different network growing methods, where our approach outperforms the current state-of-the-art.}
\label{table:main}
\end{table*}

==> tables/main_old.tex <==
\setlength{\tabcolsep}{2pt} % Default value: 6pt
\begin{table*}[t]
\resizebox{1.08\textwidth}{!}{
\centering

\begin{subtable}{0.7\linewidth}
\centering
\begin{tabular}{rlcccc}
\toprule
 & Method & CIFAR-10~\cite{Krizhevsky09learningmultiple} & CIFAR-100~\cite{Krizhevsky09learningmultiple}  &  FLOPs Norm\\ 
\midrule
 \textbf{(a)} & Target & 96.88\% & 81.39\% &  1.00X \\ 
 % \hline
 & Target Match & 96.62\% & 80.95\% &  0.45X \\ 
 % \hline
 & Seed & 96.53\% & 80.29\% &  0.25X \\
 %%% train seed model in 280 epochs
  & Seed Match & 96.60\% & 80.30\% & 0.45X \\
  \midrule
 \textbf{(b)} & Random & 95.61\% & 78.54\% & 0.45X \\
 & Firefly~\cite{wu2020firefly} & 95.62\% & 78.58\% &  0.45X \\
 & GradMax~\cite{evci2022gradmax} & 95.73\% & 78.66\% & 0.45X \\  
 & \textbf{\OurMethod\ (ours)} & \textbf{96.66\%} & \textbf{81.50\%} &  0.45X \\
 \bottomrule
\end{tabular}
\end{subtable}

\hfill

\begin{subtable}{.8\linewidth}
\centering
\begin{tabular}{rlcccc} 
\toprule
 & Method & ImageNet~\cite{deng2009imagenet} &  FLOPs Norm\\ 
\midrule
 \textbf{(a)} & Target &  76.49\% & 1.00X \\ 
 % \hline
 & Target Match & 73.85\% & 0.35X \\ 
 % \hline
 & Seed & 72.48\% & 0.25X \\
 %%% train seed model in 280 epochs
  & Seed Match & 72.89\% & 0.35X \\
  \midrule
 \textbf{(b)} & Random & 71.47\% & 0.35X \\
 & Firefly~\cite{wu2020firefly}  & 71.30\% & 0.35X \\
 & GradMax~\cite{evci2022gradmax} & 71.73\% & 0.35X \\  
 & \textbf{\OurMethod\ (ours)} & \textbf{74.51\%} & 0.35X \\
 \bottomrule
\end{tabular}
\end{subtable}
}

\caption{\textbf{Network growing performance comparison.} We compare top-1 accuracy averaged over three runs for fixed training FLOP budget on CIFAR (left) and ImageNet. \textbf{(a)} reports the performance of training the large (post-growth) \emph{Target} network architecture from scratch (WRN-28-10 for both CIFAR datasets  and ResNet-50 for ImageNet), as well as performance of the small (pre-growth) \emph{Seed} architecture (WRN-28-5 for both CIFAR datasets and a ResNet-50 with half the channels as the large network for ImageNet);  \textbf{(b)} reports the performance of different network growing methods, where our approach outperforms the current state-of-the-art.}
\vspace{-15pt}

\label{table:main}
\end{table*}



==> tables/ours_with_and_without_fusion.tex <==

\begin{table}[t]
\centering
\resizebox{\textwidth}{!}{

\begin{tabular}{lcccc} 
\toprule
 Method & CIFAR-10~\cite{Krizhevsky09learningmultiple} & CIFAR-100~\cite{Krizhevsky09learningmultiple} & ImageNet~\cite{deng2009imagenet} \\ 
\midrule
\OurMethod{}\ w/o model fusion & 96.05\% & 79.44\% & 73.02\%\\
 \textbf{\OurMethod\ (ours)} & \textbf{96.66\%} & \textbf{81.50\%} & \textbf{74.35\%}  \\
 \bottomrule
\end{tabular}
}
\vspace{6pt}
\caption{Comparison of growing using our approach with and without model fusion approach described in Section~\ref{sec:fusion} with the same FLOPs (0.45 FLOPs for CIFAR, 0.36 FLOPs for Imagenet). We find that growing by fusing together two small networks obtains a consistent boost over growing from a single small network.}
\label{table:fusion}
\end{table}


==> tables/seed_match.tex <==
\begin{table}[t]
\centering
\begin{tabular}{rlcc} 
\toprule
 Method & Top-1 Acc. &  FLOPs Norm   \\
 \midrule
 Seed 100 epochs (CIFAR10) & 94.57\% &  0.25X \\
 Seed 280 epochs (CIFAR10) & 94.92\% &  0.7X \\ % 94.88, 94.972 Total FLOPs: 3.833e+11, Total Wallclock: 02:03:46
 
\midrule
 Seed 100 epochs (CIFAR100) & 77.92\% &  0.25X \\
 Seed 280 epochs (CIFAR100) & 78.64\% &  0.7X \\ % 78.546, 78.435, 78.926 ; Total Wallclock: 01:57:46, Total FLOPs: 3.833e+11
 

 \bottomrule
\end{tabular}
\caption{Comparison growth methods under different FLOPs budgets on CIFAR-10. 
}
\label{table:horizontal_vertical}
\end{table}



==> tables/table1_cifar100.tex <==
% vgg 48.76 percent

% gradmax theirs 78.55



\begin{table}[t]
\centering
\begin{tabular}{lrr} 
\toprule
 Method & Top-1 Acc. &  FLOPs Norm   \\ [0.5ex] 
\midrule
 Target & 79.10\% &  1.00X  \\ 
 % \hline
 Target Match & 78.74\% &  0.71X  \\ 
 % \hline
 Seed & 77.65\% &  0.25X  \\
  \midrule

 %\hline
 %Full Ens. & 79.63\% & $2.738 \times 10^{11}$ & 0.50X  \\
 % \hline
 %\textbf{\OurMethod} & \textbf{78.08\%} & $2.908 \times 10^{11}$ & 0.53X \\
 % \hline
 Random & 77.83\% &  0.69X \\
 % \hline
 % \hline
 Firefly & 77.71\% &  0.69X \\
 % \hline
 % \hline
 GradMax & 77.89\% &  0.69X \\  
 % \hline 
 \midrule
 Random (gradmax schedule) & 78.16\% &  1.43X \\
 Firefly (gradmax schedule) & 78.60\% &  1.43X \\

 GradMax (gradmax schedule) & 78.55\% &  1.43X \\  
 % \hline
 \midrule
  \textbf{\OurMethodWithoutEns{}} & 78.36\% & 0.70X \\  %% Grow after 42 epochs, acc=(78.31+78.05+78.720)/3
 \textbf{\OurMethod} & \textbf{79.26\%}   & 0.70X \\
 \bottomrule
%  Ens. Rand. & 77.72\% &  $3.719 \times 10^{11}$ & - & 01:28:37 \\
%  \hline
%  Ens. Equiv. & 78.71\% & $3.719 \times 10^{11}$ & - & 01:28:37 \\
%  \hline
%  \hline
%  Depth (16-10) & - & - & $\sim 0.5$X & 01:14:54* \\
%  \hline
\end{tabular}
\caption{Results on \textbf{CIFAR-100} using a WRN 28-10 as the Target network. We grow from a WRN-28-5 size model to a WRN-28-10. \textbf{Target} refers to a WRN-28-10 trained with the same learning schedule as other methods e.g. for 100 epochs. \textbf{Seed} is a WRN-28-5 trained for 100 epochs. GradMax schedule represents a longer, 200 epoch growing schedule from the GradMax experimental setup.  We compare our to Firefly~\cite{wu2020firefly}, GradMax~\cite{evci2022gradmax}, and Random growth. MixtureGrowth outperforms even the target network, with 30 percent fewer FLOPS. This demonstrates the efficacy of our model fusing aproach for growth in template-mixing networks. All results are averaged over three runs.}
\label{table:cifar100}
\end{table}



==> tables/table2_imagenet.tex <==
\begin{table}[t]
\centering
\begin{tabular}{lrr} 
\toprule
 Method & Top-1 Acc. & FLOPs Norm  \\ [0.5ex] 
\midrule
 Target & 77.43\% &  1.00X \\ 
 % \hline
 Target Match & 76.55\% &  0.68X \\ 
 % \hline
 Seed & 70.46\% & 0.25X  \\
% \hline
% Full Ens. & 74.91\% & $2.007 \times 10^{11}$ & 0.51X  \\
 % \hline
 \hline

 Random & 71.38\%   & 0.73X  \\
 % \hline
 Firefly & 71.19\%  & 0.73X  \\
 % \hline
 GradMax & 71.66\%  & 0.73X  \\ 
 % \hline
 \midrule
\textbf{\OurMethodWithoutEns{}} & 75.46\% & 0.68X \\

 \textbf{\OurMethodEns} & 76.17\% &  0.68X  \\
 \bottomrule
\end{tabular}
\caption{Results on \textbf{ImageNet} using a ResNet as the Target network. Our method outperforms the baseline methods for a given number of training FLOPs by almost 5 percent for a given top-1 accuracy.  }
\label{table:imagenet}
\end{table}

==> tables/table3_cifar10.tex <==
% vgg 48.76 percent

% gradmax theirs 78.55



\begin{table}[t]
\centering
\begin{tabular}{lrr} 
\toprule
 Method & Top-1 Acc. &  FLOPs Norm   \\ [0.5ex] 
\midrule
 Target & 94.94\% &  1.00X  \\ % (94.962+94.952+94.892)/3
 Target Match & 94.82\% &  0.71X  \\  
 Seed & 94.66\% &  0.25X  \\  % (94.551+94.882+94.541)/3
  \midrule

 Random & 95.22\% &  0.69X \\
 Firefly & 95.37\% &  0.69X \\
 GradMax & 95.25\% &  0.69X \\  

 \midrule
 \textbf{\OurMethodWithoutEns{}} & 95.15\% & 0.70X \\  %% Grow after 42 epochs,  (95.350+95.700+94.41)/3 ~ 95.15333333333335
 \textbf{\OurMethodEns} & 95.48\%   & 0.70X \\  %  grow 63; (95.560+95.47+95.42)/3~95.48333333333333
 \bottomrule
 
\end{tabular}
\caption{Results on \textbf{CIFAR-10} using a WRN 28-10 as the Target network. We grow from a WRN-28-5 size model to a WRN-28-10. \textbf{Target} refers to a WRN-28-10 trained with the same learning schedule as other methods e.g. for 100 epochs. \textbf{Seed} is a WRN-28-5 trained for 100 epochs. GradMax schedule represents a longer, 200 epoch growing schedule from the GradMax experimental setup.  We compare our to Firefly~\cite{wu2020firefly}, GradMax~\cite{evci2022gradmax}, and Random growth. MixtureGrowth outperforms even the target network, with 30 percent fewer FLOPS. This demonstrates the efficacy of our model fusing approach for growth in template-mixing networks. Results averaged over 3 runs.}
\label{table:cifar10}

\end{table}



==> tables/when_to_grow.tex <==
\setlength{\tabcolsep}{6pt} % Default value: 6pt
\begin{table*}
\centering
\caption{\textbf{Ablation on growth points} where we stop training the second network to train the full model. \textbf{(a)} In the extreme case, we grow without training the second network, which is \OurMethodWithoutEns{}; (\textbf{b}) \OurMethod{} with different growth points. \textit{2nd Network FLOPs} is the proportion of full training schedule FLOPs that was used to train the second network. For example, 0.5 indicates we train the second network half of its full training before growth. All runs with the same total FLOPs Norm of 0.35X. Late growth where we train the full network after the second network was almost fully trained gains the best performance (boldface).} 
\begin{tabular}{lccc} 
\toprule
 Method & CIFAR-100 top-1 accuracy & ImageNet top-1 accuracy  &  2nd Network FLOPs   \\
 \midrule
   \textbf{(a)} w/o fusion  & 79.24\% &  73.02\% & 0.0 \\
\midrule
  %  \textbf{(b)} w/ fusion & 80.46\% &  73.75\% & 0.56X \\
  % & 81.08\% &  74.09\% & 0.64X \\
  % & 80.90\% &  74.16\% & 0.73X \\
  % & 81.09\% & \textbf{ 74.51}\% & 0.82X \\
  % & \textbf{81.44}\% &  74.33\% & 0.91X \\
  % & 81.27\% &  74.31\% & 1.00X \\
     \textbf{(b)} w/ fusion & 80.46\% &  73.75\% & 0.5 \\
  & 81.08\% &  74.09\% & 0.6 \\
  & 80.90\% &  74.16\% & 0.7 \\
  & 81.09\% & \textbf{ 74.51}\% & 0.8 \\
  & \textbf{81.44}\% &  74.33\% & 0.9 \\
  & 81.27\% &  74.31\% & 1.0 \\
 \bottomrule
\end{tabular}
\vspace{4pt}

\label{table:when_to_grow}
\end{table*} 

